SceneVerse: Scaling 3D Vision-Language Learning for Grounded Scene Understanding

3D vision-language grounding, which focuses on aligning language with the 3D physical environment, stands as a cornerstone in the development of embodied agents. In comparison to recent advancements in the 2D domain, grounding language in 3D scenes faces several significant challenges: (i) the inherent complexity of 3D scenes due to the diverse object configurations, their rich attributes, and intricate relationships; (ii) the scarcity of paired 3D vision-language data to support grounded learning; and (iii) the absence of a unified learning framework to distill knowledge from grounded 3D data. In this work, we aim to address these three major challenges in 3D vision-language by examining the potential of systematically upscaling 3D vision-language learning in indoor environments. We introduce the first million-scale 3D vision-language dataset, SceneVerse, encompassing about 68K 3D indoor scenes and comprising 2.5M vision-language pairs derived from both human annotations and our scalable scene-graph-based generation approach. We demonstrate that this scaling allows for a unified pre-training framework, Grounded Pre-training for Scenes (GPS), for 3D vision-language learning. Through extensive experiments, we showcase the effectiveness of GPS by achieving state-of-the-art performance on all existing 3D visual grounding benchmarks. The vast potential of SceneVerse and GPS is unveiled through zero-shot transfer experiments in the challenging 3D vision-language tasks. Project website: https://scene-verse.github.io.

==> figures/data_scale.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.49\linewidth]{ScanRefer.pdf}
    \hfill
    \includegraphics[width=0.49\linewidth]{SceneVerse-val.pdf}
    \caption{\textbf{Model performance \textit{v.s.} data scale.} Models consistently improve in both the pre-train and zero-shot transfer settings on ScanRefer and \dataset-val with data scaling-up.}
    \label{fig:data_scale}
\end{figure}%

==> figures/fig_data_generation.tex <==
\begin{figure*}[t!]
    \centering
    \captionsetup{type=figure}
        % \fbox{\rule[0cm]{0cm}{5cm}\rule[0cm]{\linewidth}{0cm}}
        \includegraphics[width=\linewidth]{figures/dataset.png}
        \captionof{figure}{
            An overview of collected data, scene graph, and important statistics.
        }
    \label{fig:data_generation}
\end{figure*}%

==> figures/fig_model.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/model.pdf}
    \caption{\textbf{Overview of our proposed \model model.} We leverage contrastive alignment in three levels $\mathcal{L}_{\text{obj}}$, $\mathcal{L}_{\text{scene}}$, and $\mathcal{L}_{\text{ref}}$ as well as a masked language modeling objective $\mathcal{L}_{\text{MLM}}$ for model learning.}
    \label{fig:model}
\end{figure}%

==> figures/fig_stats_new.tex <==
\begin{figure*}
  \begin{subfigure}{0.5\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/data_collection.pdf}
    \caption{Caption for Figure 1}
    \label{fig:figure1}
  \end{subfigure}%
  \hfill
    \begin{subfigure}{0.2\linewidth}
      \centering
      \includegraphics[width=\linewidth]{figures/scene_sanky.pdf}
      \caption{Caption for Figure 2a}
      \label{fig:figure2a}
    \end{subfigure}%
   \hfill 
    \begin{subfigure}{0.25\linewidth}
      \centering
      \includegraphics[width=\linewidth]{figures/language_starplot.pdf}
      \caption{Caption for Figure 2b}
      \label{fig:figure2b}
    \end{subfigure}
\end{figure*}


==> tables/data_ablation.tex <==
\begin{table}
    \centering
    \small
    \caption{\textbf{Ablation on scene-text pair types used in training}. We report model results on ScanRefer with no additional finetuning.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccc}
        \toprule
        Template & \acs{llm} & Anno. & Acc@0.25 & Acc@0.5\\
        \midrule
        % 3D-VisTA  & \xmark & \xmark & \xmark & \\
        % 3D-VisTA (\dataset) & & & & \\
        \xmark & \xmark & \xmark & 43.5 & 38.4 \\
        \cmark & \xmark & \xmark & 50.9 & 46.1 \\
        \cmark & \cmark & \xmark & 51.1 & 46.3 \\
        \cmark & \cmark & \cmark & 52.0 & 47.1 \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:data_ablation}
\end{table}

==> tables/model_ablation.tex <==
\begin{table}
    \caption{\textbf{Model ablation of our model on \dataset-val.}}
    \centering
    \small
    % \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccccc}
        \toprule
        Obj-lvl & MLM & Scene-lvl & Overall & Easy & Hard \\ % & V-Dep. & V-Indep.\\
        \midrule
        % 3D-VisTA  & \xmark & \xmark & \xmark & \\
        % 3D-VisTA (\dataset) & & & & \\
        \xmark & \xmark & \xmark & 64.8 & 75.4 & 48.7 \\ % & 58.3 & 72.2 \\
        \cmark & \xmark & \xmark & 65.2 & 77.1 & 47.4 \\ % & 59.2 & 72.2 \\
        \cmark & \cmark & \xmark & 62.4 & 73.4 & 45.8 \\ % & 57.7 & 67.7 \\
        \cmark & \cmark & \cmark & \textbf{66.9} & \textbf{77.8} & \textbf{50.3} \\ %& 62.6 & 71.8 \\
        \bottomrule
        \end{tabular}
    % }
    \label{tab:model_ablation}
\end{table}

==> tables/multiscan_transfer.tex <==
\begin{table}
    \centering
    \caption{\textbf{Zero-shot transfer on \dataset-val.} We evaluate models following settings in Nr3D/Sr3D using GT object proposals.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lccccc}
        \toprule
        Method & Overall & Easy & Hard & V-Dep. & V-Indep.\\
        \midrule
        3D-VisTA (\textit{scratch})  & 40.7 & 53.1 & 21.6 & 37.3 & 44.3 \\
        3D-VisTA (\textit{zero-shot})     & 52.9 & 59.6 & 35.4 & 53.7 & 52.2 \\
        3D-VisTA (\textit{zero-shot text})   & 58.1 & 70.0 & 39.6 & 52.5 & 64.1 \\
        % 3D-VisTA (finetune) & 61.4 & 74.8 & 40.9 & 56.2 & 67.1 \\
        \midrule
        Ours (\textit{scratch}) & 38.5 & 50.2 & 20.8 & 33.7 & 43.9 \\
        Ours (\textit{zero-shot}) & 59.2 & 69.4 & 44.0 & 53.1 & 66.3 \\
        Ours (\textit{zero-shot text}) & 60.6 & 70.9 & 45.1 & 54.8 & 67.3 \\
        % Ours (finetune) & 64.9 & 75.8 & 48}.5 & 58.5 & 72.3 \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:multiscan_transfer}
\end{table}

==> tables/s3d.tex <==
\begin{table}
    \centering
    \caption{Cross domain analysis for real and synthetic datasets.}
    % \resizebox{\linewidth}{!}{
        \begin{tabular}{cccccc}
        \toprule
        Real & Synthetic & ScanRefer & Structure3D\\
        \midrule
        % 3D-VisTA  & \xmark & \xmark & \xmark & \\
        % 3D-VisTA (\dataset) & & & & \\
        \cmark & \xmark &  & \\
        \xmark & \cmark & & \\
        \cmark & \cmark & & \\
        \bottomrule
        \end{tabular}
    % }
    \label{tab:s3d_comparison}
\end{table}

==> tables/scannet_transfer.tex <==
% \begin{table}
%     \centering
%     \caption{Zero-shot and supervised transfer on existing benchmarks.}
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{ccccc}
%         \toprule
%         Method & ScanRefer & Nr3D & Sr3D & MultiScan\\
%         \midrule
%         3D-VisTA (scratch) & 41.5 & 57.5 & 69.6 & \\
%         3D-VisTA (zero) & & & & \\
%         3D-VisTA (w/ sgrefer) & & & & \\
%         3D-VisTA (finetune) & & & & \\
%         \midrule
%         Ours (scratch) & & & & \\
%         Ours (zero) & & & & \\
%         Ours (w/ sgrefer) & & & & \\
%         Ours (finetune) & & & & \\
%         \bottomrule
%         \end{tabular}
%     }
%     \label{tab:supervised_transfer}
% \end{table}

\begin{table}
    \centering
    % \small
    \caption{\textbf{Zero-shot transfer results on established benchmarks.}}
    % ``ScanRefer@k'' stands for ScanRefer evaluation with IoU@$k$.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccc}
        \toprule
        Method & Nr3D & Sr3D & ScanRefer@0.25 & ScanRefer@0.5\\
        \midrule
        3D-VisTA (\textit{scratch}) & 57.5 & 69.6  & 45.9 & 41.5\\
        3D-VisTA (\textit{zero-shot}) & 35.2 & 31.2 & 33.2 & 29.6 \\
        3D-VisTA (\textit{zero-shot text}) & 43.1 & 36.1 & 41.1 & 36.4 \\
        % 3D-VisTA (finetune) & 50.0 & 44.9 & & \\
        \midrule
        Ours (\textit{scratch}) & 58.7 & 68.4 & 44.5 & 40.4 \\
        Ours (\textit{zero-shot}) & 32.4 & 33.3 & 35.2 & 31.1  \\
        Ours (\textit{zero-shot text}) & 41.9 & 38.1 & 40.7 & 35.8 \\
        % Ours (finetune)     & 50.2 & 45.4 &  59.8 & 71.5 \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:scannet_transfer}
\end{table}

==> tables/scanqa.tex <==
\begin{table}
    \centering
    \small
    \captionof{table}{\textbf{3D question answering results on ScanQA and SQA3D.} We report EM@1 score on all ScanQA and SQA3D.}
    \begin{tabular}{ccccccc}
    \toprule
    Model & EM@1 & EM@10 & BLEU-4 & ROUGE & METEOR & CIDEr \\
    \midrule
    Image+MCAN & 22.3 / 20.8 & 53.1 / 51.2 & 14.3 / 9.7 & 31.3 / 29.2 & 12.1 / 11.5 & 60.4 / 55.6 \\
    ScanRefer+MCAN & 20.6 / 19.0 & 52.4 / 49.7 & 7.5 / 7.8 & 30.7 / 28.6 & 12.0 / 11.4 & 57.4 / 53.4 \\
    ScanQA & 23.5 / 20.9 & 56.5 / \textbf{54.1} & 12.0 / 10.8 & 34.3 / 31.1 & 13.6 / 12.6 & 67.3 / 60.2 \\
    3D-VisTA & \textbf{27.0} / 23.0 & \textbf{57.9} / 53.5 & \textbf{16.0} / 11.0 & \textbf{38.6} / \textbf{32.8} & \textbf{15.2} / \textbf{12.9} & \textbf{76.6} / \textbf{62.6} \\
    3D-LLM & 19.1 / - & - / - &  11.6 / - & 35.3 / - & 14.9 / - & 69.6 / -\\
    \midrule
    Ours & 25.0 / \textbf{23.5} & 54.6 / 52.9 &  14.5 / \textbf{13.7} & 35.0 / 32.1 & 13.6 / 12.5 & 68.0 / 61.0 \\
    \bottomrule
    \end{tabular}
    \label{tab:scanqa}
\end{table}

==> tables/scanrefer.tex <==
% \begin{table*}
%     \centering
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{ccccccc}
%         \toprule
%         \multirow{2}[2]{*}{Method} & \multicolumn{2}{c}{Unique Acc} & \multicolumn{2}{c}{Multiple Acc} & \multicolumn{2}{c}{Overall Acc}\\
%         \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
%         & @0.25 & @0.5 & @0.25 & @0.5 & @0.25 & @0.5\\
%         \midrule
%         3DVG-Trans~\cite{zhao20213dvg} & 81.9 & 60.6 & 39.3 & 28.4 & 47.6 & 34.7 \\
%         3D-SPS~\cite{luo20223d} & 84.1 & 66.7 & 40.3 & 29.8 & 48.8 & 37.0 \\
%         3DJCG~\cite{cai20223djcg} & 83.5 & 64.3 & 41.4 & 30.8 & 49.6 & 37.3 \\
%         SAT~\cite{yang2021sat} & 73.2 & 50.8 & 37.6 & 25.2 & 44.5 & 30.1 \\
%         MVT~\cite{huang2022multi} & 77.7 & 66.5 & 31.9 & 25.3 & 40.8 & 33.3 \\
%         ViL3DRel~\cite{chen2022language} & 81.6 & 68.6 & 40.3 & 30.7 & 47.9 & 37.7 \\
%         BUTD-DETR~\cite{jain2022bottom} & 82.9 & 65.0 & 44.7 & 34.0 & 50.4 & 38.6 \\
%         EDA~\cite{wu2023eda} & 85.8 & 68.6 & 49.1 & 37.6 & 54.6 & 42.3 \\
%         3D-VisTA~\cite{zhu20233d} & 81.6 & 75.1 & 43.7 & 39.1 & 50.6 & 45.8 \\
%         \midrule
%         Ours & & & & & & \\ 
%         \bottomrule
%         \end{tabular}
%     }
% \end{table*}

\begin{table*}
    \centering
    \caption{3D visual grounding results on ScanRefer \bx{might need to toggle acc@0.25 for visualization}}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ccccccccc}
        \toprule
        \multirow{2}[2]{*}{Method} & \multirow{2}[2]{*}{Modality} & \multirow{2}[2]{*}{3D-Det.} & \multicolumn{2}{c}{Unique} & \multicolumn{2}{c}{Multiple} & \multicolumn{2}{c}{Overall}\\
        \cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
        & & & Acc@0.25 & Acc@0.5 & Acc@0.25 & Acc@0.5 & Acc@0.25 & Acc@0.5\\
        \midrule
        3DVG-Trans~\cite{zhao20213dvg} & 3D+2D & Opt. & 81.9 & 60.6 & 39.3 & 28.4 & 47.6 & 34.7 \\
        SAT~\cite{yang2021sat} & 3D+2D & VN & 73.2 & 50.8 & 37.6 & 25.2 & 44.5 & 30.1 \\
        3D-SPS~\cite{luo20223d} & 3D+2D & Opt. & 84.1 & 66.7 & 40.3 & 29.8 & 48.8 & 37.0 \\
        3DJCG~\cite{cai20223djcg} & 3D+2D & Opt. & 83.5 & 64.3 & 41.4 & 30.8 & 49.6 & 37.3 \\
        MVT~\cite{huang2022multi} & 3D+2D & PG & 77.7 & 66.5 & 31.9 & 25.3 & 40.8 & 33.3 \\
        BUTD-DETR~\cite{jain2022bottom} & 3D & Opt. & 82.9 & 65.0 & 44.7 & 34.0 & 50.4 & 38.6 \\
        ViL3DRel~\cite{chen2022language} & 3D & PG & 81.6 & 68.6 & 40.3 & 30.7 & 47.9 & 37.7 \\
        EDA~\cite{wu2023eda} & 3D & Opt. & 85.8 & 68.6 & 49.1 & 37.6 & 54.6 & 42.3 \\
        3D-VisTA~\cite{zhu20233d} & 3D & M3D & 81.6 & 75.1 & 43.7 & 39.1 & 50.6 & 45.8 \\
        \midrule
        Ours & 3D & M3D & & & & & & \\ 
        \bottomrule
        \end{tabular}
    }
    \label{tab:scanrefer}
\end{table*}

==> tables/synthetic_dataset.tex <==
\begin{table}
    \centering
    \caption{\textbf{Cross domain transfer results} of models learned in real and synthetic datasets without additional fine-tuning. ``S3D'' stands for Structured3D.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{ccccc}
        \toprule
        Real & Synthetic & \dataset-val & S3D & ProcTHOR\\
        \midrule
        % 3D-VisTA  & \xmark & \xmark & \xmark & \\
        % 3D-VisTA (\dataset) & & & & \\
        All & \xmark & 64.8 & 37.1 & 43.4 \\
        \xmark & S3D & 7.0 & 85.1 & 16.1 \\
        \xmark & ProcTHOR & 4.2  & 16.3 & 91.0 \\
        % \cmark & \cmark & & \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:synthetic_dataset}
\end{table}

==> tables/zero_shot_semantic_seg.tex <==
\begin{table}
    \caption{\textbf{Semantic segmentation results on ScanNet validation set.} }
    \centering
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lccc}
        \toprule
        Method                                  & Backbone                          & mIoU$^{\dagger}$              & mAcc$^{\dagger}$          \\ \hline
        PLA$^{\ddagger}$                        & SparseUNet16~\cite{graham20183d}  & 17.7                          & 33.5                      \\ \hline
        OpenScene-3D~\cite{peng2023openscene}   & MinkowskiNet18A~\cite{choy20194d} & 56.7                          & 68.3                      \\ \hline
        OpenScene-3D$^{\ddagger}$~\cite{peng2023openscene}   & SparseUNet16~\cite{graham20183d}  & 57.2              & 69.9                      \\ \hline
        RegionPLC~\cite{yang2023regionplc}      & SparseUNet16~\cite{graham20183d}  & 56.9                          & 75.6                      \\ \hline
        Ours                                    & SparseUNet16~\cite{graham20183d}  & 52.5                          & 73.1                      \\ \hline
        Ours                                    & Res16UNet34C~\cite{choy20194d}                      & 55.6                          & 76.1                      \\ \hline
        \bottomrule
        \end{tabular}
    }
    \label{tab:zero_shot_semantic_seg}
\end{table}

==> tables/zeroshot_transfer.tex <==
\begin{table}
    \centering
    \caption{Zero-shot transfer results on MultiScan and Scan-Net.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccc}
        \toprule
        Method & ScanRefer & Nr3D & Sr3D & MultiScan  \\
        \midrule
        3D-VisTA & & & & \\
        \midrule
        Ours & & & & \\
        \bottomrule
        \end{tabular}
    }
    \label{tab:zeroshot_transfer}
\end{table}
